How Far Are We? The Triumphs and Trials of Generative AI in Learning Software Engineering

Conversational Generative AI (convo-genAI) is revolutionizing Software Engineering (SE) as engineers and academics embrace this technology in their work. However, there is a gap in understanding the current potential and pitfalls of this technology, specifically in supporting students in SE tasks. In this work, we evaluate through a between-subjects study (N=22) the effectiveness of ChatGPT, a convo-genAI platform, in assisting students in SE tasks. Our study did not find statistical differences in participants' productivity or self-efficacy when using ChatGPT as compared to traditional resources, but we found significantly increased frustration levels. Our study also revealed 5 distinct faults arising from violations of Human-AI interaction guidelines, which led to 7 different (negative) consequences on participants.

==> _tex_folder/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> _tex_folder/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> sec/TODO.tex <==
Link to the rebuttal doc: 
https://docs.google.com/document/d/1TDwC0-yj2BBKlFH0mcuE-YJKxmBfh_JEr3xmtS-xW_4/edit 

Problem with putting A statement in beginning of results:
- Half of conclusion is shifting to page 11.

==> sec/intro-copy.tex <==
\section{Introduction (BUD 1.25 PAGE)}
\label{sec:intro}
% Story:
% **Convo-genAI is all the craze, including ed....
% ** Past work has shown
% 1) how convo agents are helpful
% 2) how genAI is helpful
% ** But all of this is for intro CS, what about higher division courses
% ** SE is one such, has more complex...convo+genAI tools can be helpful in giving context help
% ** Thus, we do blah
% **


\boldification{convo GenAI discussions go both ways, we dont know how SE ed can leverage GenAI.}
The advent of Conversational Generative AI (convo-genAI) is proving to be a ``Gutenberg moment'' across education and business, including in software engineering. These systems (e.g, ChatGPT \cite{GPT4}, Google Bard \cite{bard}, Meta LLaMA\cite{llama}) can generate new contextualized content, be it a  haiku or a relevant code snippet, informed by pre-existing data and minimal input. Additionally, these tools provide a conversational interface, enabling users to interactively engage with it using natural language to generate outputs fine-tuned to their requirements. Discussions on the use of generative AI range from how it signals the ``end of programming'' \cite{welsh2022end, yellin2023premature} to how it can transform software engineering for the better \cite{daun2023chatgpt, ma2023scope}. 
Given the nascency of this innovation, it remains unclear how software engineering can fully leverage it in education and uncertainty shadows its potential benefits.

\boldification{Introductory CS education has investigated conversational agents and GenAI}
Introductory Computer Science (CS) education has investigated both conversational agents and GenAI.
% Conversational interfaces allow users to dialog in natural language have been studied in the context of CS education. 
Prior work on conversational agents has demonstrated their effectiveness for non-specialists and learners, as it facilitates dialogue with an "expert" \cite{ritzel2019development, valtolina2020communicability, walgama2017chatbots, grudin2019chatbots}. For example, Loksa et al. \cite{loksa2016programming} found that high-schoolers in an introductory programming-summer camp benefitted when they could seek help by articulating their problem solving strategies and its state.  
Further, the new generation of students have been found to prefer talking with chatbots over talking to a person \cite{alton2017phone, murtarelli2023hi}. Indeed, there has been extensive work on conversational agents for education \cite{Okonkwo2021chatbots, wollny2021we} that focuses on students’ engagement \cite{benotti2014engaging,bii2013chatbot,fryer2017stimulating}, self-directed learning \cite{pereira2016leveraging}, and tutoring \cite{tamayo2017designing}. 

Research on introductory CS education has also explored the use of genAI systems~\cite{denny2022robosourcing, macneil2022generating, verleger2018pilot}. %as well as a pair programming buddy for  developers\cite{bird2022taking}. 
% \citet{verleger2018pilot} investigated the use of AI-driven chatbot to [result] use in problem solving. Similarly, \citet{macneil2022generating} looked into how these systems can be leveraged for generating code explanations. 
But these works have either been focused on using genAI to solve algorithmic problems \cite{peng2023impact,sun2022investigating} (i.e., focus on programming) or on improving genAI technology and output \cite{li2023blip,white2023prompt} (i.e., focus on better AI).

\boldification{thus far, no one has looked at genAI in SE courses, which are particularly suited for this}
Currently, there is a gap in understanding how convo-genAI systems can be leveraged for upper-division CS education, such as Software Engineering (SE), where the learning objectives include unique complexities (concepts, processes, tools) and contextual decision making involving subjectivity and multiple trade-offs \cite{pinto2017training, pinto2019training}. Each of these situations are unique and require contextualized assistance.
Given that these AI systems are now capable of providing such assistance, coupled with natural language dialogue capabilities, it can be particularly well suited in teaching SE topics \cite{daun2023chatgpt}, in which traditional chatbots have fallen short so far\cite{farooq2016human, dominic2020conversational}). 
%
% But we dont know how and in what capacity would using convo-gen-AI best support SE students. how they will interact with the agent to get to the right solution and how the technology helps or impedes their efficiency and self confidence.
Therefore, it is essential to have a clear understanding of where and to what extent these systems can be helpful in software engineering education. 

\rudy{This paragraph needs attention. I feel like we are repeating stuff.}
In this paper, we first ask:
\textbf{\textit{(RQ1): How effective is convo-genAI in helping students in software engineering?}} Specifically we investigated how well it is in assisting students with SE concepts (fixing code functionalities, good coding practices), processes and tools.
%
We answered this research question through a between-subjects user study, where the Experimental Group solely used ChatGPT, while participants in the Control Group could use any resource other than Generative AI tools.
We selected ChatGPT as a representative convo-genAI as it is the state-of-the-art at the time of writing this paper. We recruited 22 students who had recently completed or were currently enrolled in undergraduate software engineering courses at our university. Participants in both groups completed three SE tasks (fixed code functionalities, removed code smells, contributed their changes to an open source repository).  
We found no statistical differences between the two treatments in terms of participants' task performance or overall self-efficacy, but using ChatGPT did increase participants' frustration.

Furthermore, to gain a comprehensive understanding of how Convo-GenAI can be effectively used and to inform its future design, it is essential to identify and evaluate its current pitfalls.
This leads to our second research question:
\textit{\textbf{(RQ2): What are the current pitfalls in convo-genAI?}} 
Specifically, what are the faults that convo-genAI currently makes? What causes these faults and what are its consequences on the students?
To answer this question, we employed After-Action Review for AI (AAR/AI) \cite{dodge-aar}, a recent AI assessment process that allows end users in gauging AI faults \cite{khanna2022finding} through a set of questions (see Section~\ref{subsubsec: instruments}). The purpose of using AAR/AI was to assess the faults that participants (in the experimental group) could perceive during their interaction with ChatGPT as well as its consequences for the participants. A qualitative analysis of these responses revealed 5 distinct categories of faults and 7 distinct consequences stemming from these faults. Additionally, we used Microsoft's design guidelines for Human-AI Interaction (HAI) \cite{amershi2019guidelines} as a lens to track which of these faults were a result of violating specific guidelines.
We harvested (Experimental Group) participants' feedback on their perceptions of whether any of the HAI Guidelines were violated by ChatGPT in a post-study likert-scale questionnaire. 
They reported that ChatGPT: (1) did not clearly outline its capabilities and limitations, (2) did not support efficient correction, (3) did not scope itself when in doubt, and (4) lacked transparency its decision making process. Our analysis revealed that these guideline violations were a root cause of the identified faults.
% Future design should address these violations to better tailor genAI systems for improved human-AI interaction.

% Delving into these issues will not only guide appropriate usage in the present but also inform the future design of Generative AI systems, with a focus on enhancing human-AI interaction

\rudy{need sunset}
% These insights not only provide guidance for appropriate current usage but also inform the future design of Generative AI systems tailored for improved human-AI interaction. 
\boldification{ Closing statement}
Through this study, we provide a comprehensive evaluation of the potentialities and challenges of conversational Generative AI in software engineering education, highlighting its current pitfalls and simultaneously informing its future design. These insights will not only guide appropriate usage in the present but also inform the future deign of genAI systems, with a focus on enhancing human-AI interaction.

==> sec/leftover-text.tex <==
INTRODUCTION TEXT
\section{Introduction (BUD 1.25 PAGE)}
\label{sec:intro}
\boldification{ OSS is an important platform for SE education. Learning is a top motivator for contributing to OSS. }
Open Source Software (OSS) is a relevant economic driving force providing systems used through the entire development stack, from operating system kernels to sophisticated end-user applications. In addition to its business value, OSS is an important platform for education \cite{o2003open}. The primary factor that attracts newcomers to OSS is the opportunity to learn \cite{ bonaccorsi2003altruistic, alexander2002working,lakhani2005perspectives,singh2012newcomer, von2003community, silva2020google, gerosa2021shifting}. In a recent survey, learning was ranked as a top motivation for contributors to join and stay in OSS \cite{gerosa2021shifting}. David and Shapiro \cite{david2008community} show that a large number of young developers join OSS projects to improve their programming and other software engineering skills. These newcomers, who the authors call “social learners'', are particularly drawn to communities that include other newcomers from the same population (peer parity). The survey conducted by Arjona-Reina et al. \cite{arjona2014floss2013} corroborates these findings: the two dominant reasons for contributing to OSS are “sharing knowledge and skills'' and “learning and developing new skills.” Fang and Neufeld \cite{fang2009understanding} show that situated learning is also positively linked to retaining newcomers to OSS. 
% Furthermore, a recent survey conducted in 2021 showed that learning is a top-ranked motivation for contributors to join and stay in OSS \cite{gerosa2021shifting}.

\boldification{Instructors want to use OSS as a training ground for students to gain experience with real Software dev problems. Students and instructors report clear benefits of this activity.}
It is not surprising, therefore, that several software engineering educators want to use OSS projects as a training ground for students to gain experience with real software development problems, with the added benefit that students contribute to the evolution of projects relevant to society \cite{silva2020google, pinto2017training, pinto2019training, ferreira2018students, huang2021leaving}. Past research has investigated how instructors \cite{pinto2017training} and students \cite{pinto2019training} perceive the benefits and difficulties of using OSS contribution as an activity in software engineering courses. Students and instructors report clear benefits of this activity, including improving students’ social and technical skills. In addition, students and instructors found it extremely important to engage with open source initiatives. 

\boldification{ However, there are many challenges in OSS. Without appropriate support, students lose motivation. Also due to challenges educators give up on OSS activities in their courseware. }
However, it is well-known that students onboarding to OSS face many difficulties and are often left to learn on their own \cite{scacchi2002understanding, steinmacher2019overcoming}. These newcomers usually need maps and signs to support their first steps in the project landscape\cite{steinmacher2016overcoming}. 
% They are akin to explorers who must orient themselves in a hostile landscape . 
Past work has identified the challenges from feedback from students who attempted to onboard to OSS projects \cite{steinmacher2012recommending, pinto2019training}. Without appropriate support, students become demotivated, consume already scarce community resources, and become frustrated and quit. Due to these challenges, many educators give up on using contributions to OSS as an activity in their software engineering courses \cite{pinto2017training}.

\boldification{There have been efforts in literature to reduce the barriers. Nevertheless, students still face barriers as not everyone solves problems the same way.}
A more comprehensive study \cite{steinmacher2015social} classifies challenges faced by newcomers when making their first contributions. Based on this model, Steinmacher et al. designed FLOSScoach \cite{steinmacher2016overcoming}, a web portal to better orient students and OSS newcomers on how to contribute to projects, organizing the information into a coherent process that includes activities such as learning about the project and skills, setting up a local workspace, finding a task to start with, etc. The study showed that the web portal made students feel oriented and more comfortable making their first contribution. Nevertheless, students still face barriers \cite{guizani2022debug, guizani2021long} and often fail to find information in the portal or project documentation, given the different pathways they follow to make their contributions \cite{yue2022off}.

\boldification{Studies have shown that chatbots are helpful as they provide expert advice contextualized to needs. Students prefer chatbots over humans.}
Previous literature indicates that conversational interfaces may be particularly effective for non-specialists and learners seeking information by providing expert advice contextualized to their need \cite{ritzel2019development, valtolina2020communicability, walgama2017chatbots, grudin2019chatbots}. Loksa et al. \cite{loksa2016programming} showed that assisting inexperienced programmers increases productivity, independence, programming self-efficacy, metacognitive awareness, and growth mindset. The new generation of students is familiar with conversational agents and often prefers to talk to a chatbot over talking to a person \cite{alton2017phone, murtarelli2023hi}.
\boldification{ Echoing this need, there has been extensive work in the field of conversational agents for education. However, the field remains underexplored as a means of supporting software engineering students. }	
Echoing this need, there has been extensive work in the field of conversational agents for education \cite{Okonkwo2021chatbots, wollny2021we} focused on students’ engagement \cite{benotti2014engaging,bii2013chatbot,fryer2017stimulating}, self-directed learning \cite{pereira2016leveraging}, and tutoring \cite{tamayo2017designing}. However, conversational agents are still relatively underexplored as a means of supporting software engineering students to engage with open source \cite{dominic2020conversational,serrano2021find}.
% , which might be attributed to the absence of a flexible dialog management framework that facilitates intelligent interactions  \cite {farooq2016human, dominic2020conversational}.

\boldification{ Advent of GenAI: Hot topic but since it is recent, uncertainty shadows its benefits.}
The advent of Generative AI\footnote{Generative AI is a type of artificial intelligence that learns from existing data to generate new and unique outputs \cite{generativeai,bloomberglawCheatSheet}. ChatGPT and Google Bard are notable examples of generative AI for text and GitHub Copilot for code. These generative AI systems leverage large language models, such as GPT-4, LaMDA, and Codex.} is proving to be a ``Gutenberg moment'' across education and business, and software engineering is no exception. Discourse on this topic also appears in academic publications, including in recent articles in the Communications of the ACM (Association for Computer Machinery) entitled "The End of Programming" \cite{welsh2022end} and "The Premature Obituary of Programming" \cite{yellin2023premature}. However, as Generative AI is a recent innovation, it remains unclear how software engineering can fully leverage the technology in education and work, and uncertainty shadows its potential benefits.

\boldification{Current efforts are either focused on programming, or better AI, but without the understanding of this new form of AI-supported software engineering, all of it is ad-hoc}
Current research efforts have focused on using generative AI to solve algorithmic problems \cite{peng2023impact,sun2022investigating} (i.e., focus on programming) or on improving generative AI technology and output \cite{li2023blip,white2023prompt} (i.e., focus on better AI), which undoubtedly will happen given the massive investment from industry. But there is a fundamental gap in understanding how this new form of AI can support software engineering education, allowing students to engage with the technology and learn at their own pace and style.
% But there is a gap in a fundamental understanding of how this new form of AI can support software engineering education, and without this, no ``automatic programming'' can succeed \cite{meyer2022}.

\as{there is a gap in understanding how this new potential can be leveraged as scaffolding agents to improve SE education, allowing people to engage with the genAI and learn at your own paces and style. To close this gap we ...}

\rudy{But there is a gap in a fundamental understanding of how this new form of AI can support software engineering education, allowing students to engage with the technology and learn at their own pace and style.}

\boldification{To close this gap we did ...}
To close this gap, we investigated how the profound potential of Generative AI can be leveraged as conversational scaffolding agents to support students in learning software engineering. 
We specifically selected ChatGPT for this study, as it was the state-of-the-art.
%due to its acclaim and proficiency in understanding complex conversational contexts and generating human-like responses, thus fostering an intuitive and interactive environment. 
We designed our research questions (RQs) to guide our efforts in investigating:

\textit{\textbf{RQ1: How effective is Generative AI (ChatGPT) in helping students contribute to an OSS project?}}
With this question, we wanted to assess its current potentialities towards supporting students contribute to open source. We determined the effectiveness of Generative AI in our context by comparing how students $(N = 22)$ perform software engineering tasks to contribute to a toy OSS repository with and without ChatGPT. We followed a between-subjects study design (the experimental group solely used ChatGPT, while the participants in the control group were free to use any resource other than Generative AI tools). Specifically, we investigated users' perceived cognitive load \cite{hart1988development, sanneman2022situation, rosenfeld2021better, anderson2020mental}, the effects on users' productivity \cite{xu2022ide} and self-efficacy \cite{Bandura_1986}, and also their intention for future use. \textbf{We hypothesized that .... and we found that .... <to be filled after result section>}. 

\boldification{ To understand how GenAI can support, it is crucial to understand the current pitfalls. These insights will be useful for future design. Thus we investigate RQ2.}
Furthermore, to fundamentally understand how Generative AI can support software engineering education, it is imperative to unveil Generative AI itself in terms of its current pitfalls, which is essential for evaluating its behavior.
%(attributed to how it is designed), while simultaneously assessing whether its behavior differs based on user interaction nuances, indicating how AI outcomes vary based on human engagement strategies. 
These insights will not only provide guidance for appropriate current usage but also inform the future design of Generative AI systems tailored for improved human-AI interaction. Thus we assessed:

 \rudy{reflection and meta cognition - How do students actually reflect back on using Gen AI in their work}
\textit{\textbf{RQ2: What are the faults that Generative AI (ChatGPT) currently makes? What causes these faults and what are its consequences on the students?}}

\rudy{Does it seem right?}
In 1994, Nelson et al. \cite{nelson1994investigate} stated that reflecting on perception is critical for decision-making and learning. In our context, we posit that reflecting on the faults of a scaffolding agent can potentially inform and support decisions regarding its appropriate usage. 

 To that end, we employed After-Action Review for AI (AAR/AI) \cite{dodge-aar}, a recent AI assessment process that is focused on supporting end users in gauging AI faults \cite{khanna2022finding}. The purpose of using AAR/AI was to assess the faults that participants (in the experimental group) could perceive during their interaction with ChatGPT and its consequences for the participants. Upon analysis of the AAR/AI results (open coding), we identified 5 distinct categories of faults and 7 distinct consequences that arose from these faults. Furthermore, to inform future design, it is imperative to understand why these faults occurred. We used Microsoft's design guidelines for Human-AI Interaction \cite{amershi2019guidelines} as our lens and found that these faults can be attributed to  guideline violations during ChatGPT's design. 

% \rudy{removing this}
% \textit{\textbf{RQ3: How ChatGPT operates based on how it is prompted? Is prompt engineering really a thing: does it effect RQ1 and RQ2?}}
% As per a keynote talk in ICSE 2023, 
% \textit{"Every time we “prompt program” a large language model to complete a task, we create a customized version of the language model, which exhibits different abilities and outputs than other customized versions."} \footnote{Testing Generative Large Language Model: Mission Impossible or Where Lies the Path? \url{https://conf.researchr.org/details/icse-2023/deeptest-2023-papers/6/Testing-Generative-Large-Language-Model-Mission-Impossible-or-Where-Lies-the-Path-}}

% To investigate the same, we analyzed the interaction logs from our recorded sessions and classified the prompts based on whether they (helped/hindered) the participants. \textbf{Once done, how RQ1 and RQ2 differed based on the participants' interaction styles. We found ... <results section> To that end we present some good interaction styles on how to better use the tool>}

\boldification{ Closing statement}
Through this study, we provide a comprehensive evaluation of the potentialities and challenges of Generative AI in software engineering education, highlighting its current pitfalls and simultaneously informing its future design.





% Background of AAR/AI

% \boldification{What is AAR/AI and where is it adapted from?}
% \textbf{AAR/AI}: After-Action Review for AI (AAR/AI) \cite{dodge-aar} is a recent AI assessment process that is focused on supporting humans in gauging AI faults \cite{khanna2022finding}. 
% It is a recent member of the After-Action Review (AAR) family which was originally devised by the U.S. military in the 1970s \cite{morrison1999foundations} as a facilitated debriefing method for assessing human decisions during military training sessions. The AAR method has been used for decades and has subsequently been adapted to different domains including manned unmanned teams \cite{brewer2020assessment} , emergency response \cite{davies2019enhancing, ishak2017slides}, transportation \cite{baird1999learning}, and healthcare \cite{quarles2013experiences, sawyer2013adaptation}. Most of the adaptations have been successful and a meta analysis of 61 studies has found that the AAR method produces a practical moderate effect overall \cite{keiser2021meta}. 

% \boldification{ Why did we care? Did studies show that humans assess AI better with AAR/AI?}
% AAR/AI is a form of retrospective analysis and reflection to understand what happened, why it happened, and how it can be improved. It is tailor made as an assessment method for a human assessor to judge an AI (review/learn AI’s behavior). Khanna et al. \cite{khanna2022finding} provided empirical evidence that the integration of AAR/AI can aid end users in uncovering not only a significantly larger number of faults, but also in identifying these faults with greater precision. Drawing from Dodge et al. \cite{dodge-aar}, participants using AAR/AI reported that it assisted in better organization of their thoughts and fostered logical reasoning about the AI agent. Moreover, it also encouraged them to reason about the AI and its behavior from a diverse set of perspectives.

RQ3:

% \rudy{removing this}
% \textit{\textbf{RQ3: How ChatGPT operates based on how it is prompted? Is prompt engineering really a thing: does it effect RQ1 and RQ2?}}
% As per a keynote talk in ICSE 2023, 
% \textit{"Every time we “prompt program” a large language model to complete a task, we create a customized version of the language model, which exhibits different abilities and outputs than other customized versions."} \footnote{Testing Generative Large Language Model: Mission Impossible or Where Lies the Path? \url{https://conf.researchr.org/details/icse-2023/deeptest-2023-papers/6/Testing-Generative-Large-Language-Model-Mission-Impossible-or-Where-Lies-the-Path-}}

% To investigate the same, we analyzed the interaction logs from our recorded sessions and classified the prompts based on whether they (helped/hindered) the participants. \textbf{Once done, how RQ1 and RQ2 differed based on the participants' interaction styles. We found ... <results section> To that end we present some good interaction styles on how to better use the tool>}

Discussion:
% \textit{\textbf{Diverse violations for diverse users}}: Previous literature highlights that user interactions and experiences with AI systems are significantly diverse for diverse users \cite{anderson2021diverse, lee2000can, seaborn2021measuring}.
% There are often embedded gender biases in technology, that arises due to a lack of support for cognitive diversity \cite{padala2020gender}. Research spanning a decade has identified that women are more risk-averse than men \cite{charness2012strong, dohmen2011individual} and prefer process-oriented learning and are thus less likely to tinker \cite{beckwith2006tinkering, burnett2010gender, hou2006girls}.

% We found considerable disparities in perceived violations of the HAI guidelines on disaggregating participants’ data based on their gender. All women reported a violation of Guideline 11, perceiving that it was hard to gain an explanation behind ChatGPT’s decision-making process, whereas only 3 out of 6 men reported this violation. This is likely because women were more risk-averse towards using an AI-provided solution and needed more explanation about how it was derived. 
% A majority of men (5 out of 6) found that ChatGPT did not allow for global customization of its behavior (Guideline 17 violation), likely because of the limited tinkering allowed around its interface and technology. In contrast, no women found this guideline to be in violation. Similarly, 4 out of 6 men marked that ChatGPT did not personalize their experience by learning from their actions over time (Guideline 13 violation). No women reported this violation.
% We further disaggregated the data by participants' AI familiarity and experience with software engineering, but we did not find any significant patterns. More research is needed to understand how participants' familiarity with the domain and with AI can influence their interactions with and perceptions of the technology.

==> sec/old-method.tex <==
\section{Methodology}
\label{sec:method}


\subsection{Research Design}
\label{subsec:study design}
\boldification{Our research design is a between subjects design (CG vs non-LLM) and the different stages of the study design are…}
Our overall research design is illustrated in Fig. 1. We implemented a between-subjects study design wherein the experimental group was provided with ChatGPT for the tasks, while the control group was allowed to utilize any online resources with the exception of large language models. The rationale was to assess GenAI’s assistance, in the form of ChatGPT, in comparison to more traditional online resources. The initial phase of the study design involved understanding our participant population, which subsequently informed our task design. This was followed by selecting our analytical lenses to address the research questions effectively. Subsequently, we carried out six sandboxing phases with students, making necessary amendments to the study design as required. These modifications were implemented following discussions and consensus within the research team. Following this iterative refinement process, we recruited our actual study participants, and filtered the pool to ensure eligibility in line with our research criteria. The study was then conducted in-person at the university lab and spanned a period of three weeks. 

\begin{table}[h]
\vspace{-6pt}
 \caption{\small{Metrics and instruments.}} % title of Table
 \label{table:metrics} % is used to refer this table in the text
 \vspace{-8pt}
% \centering
\input{table/Metrics-Instruments}
\vspace{-15pt}
\end{table}


\boldification{ We start with knowing our participant population. To achieve that we had a meeting with a course instructor and identified what our participants were familiar with, which informed our task design.}

\textit{Designing the tasks}: The crucial part of designing the right tasks is to correctly assess the participant population. To that end, three researchers had an online meeting with the course instructor of a Software Engineering course at the university. From the discussion, we identified that the students had low to medium familiarity with Git and GitHub, and the common programming languages used in the course were Python and Javascript. Furthermore, we discussed that the students were novices in Software Engineering and had rudimentary understanding of good programming styles, API usage, and web scraping. These informed our task design for the study. 

\boldification{ After the initial discussion, the team came up with the study tasks (what are they) and iteratively revised it. The tasks were of moderate complexity (why)}
After the initial discussion, the research team held online meetings over two weeks, where the tasks were continually reviewed and rearranged. Our goal was to evaluate the helpfulness of the resources (eg: ChatGPT), so the tasks were designed to be moderately challenging for software engineering novices. Ultimately, we developed three tasks centered on contributing to a toy GitHub repository. We chose Python as the programming language for this exercise. The selection and sequencing of these three tasks were thoughtfully designed to mimic a typical contribution scenario that involves contributors creating their own branch, rectifying the code, addressing code smells or standardizing the code style, and finally contributing their changes back to the project by opening a PR. In an effort to increase the complexity for code comprehension so as to realistically simulate a common software engineering challenge, we intentionally obfuscated the code. This was achieved by disorganizing the code structure, incorporating poorly crafted comments, and employing unintuitive function names. These adjustments were designed to introduce a moderate level of challenge in understanding and interpreting the code.

\boldification{ The first task was ….}
\textit{Task 1:} In the first task, participants needed to create their own git branch and fix the code functionalities in their branch so as to pass three test cases. They were restricted from modifying the main method or creating their own test cases. The three test cases were set as follows: (1) In the first test case, participants had to correct a function that checked if a number was a palindrome. We intentionally reversed the logic of this function, creating a bug for the participants to fix. (2) For the second test case, participants were tasked with correcting a function termed 'check\_weather'. The objective of the function was to retrieve weather data using the NOAA\_SDK library \cite{NOAA} in Python, given specific latitude and longitude coordinates. The correct method for this operation would have been to utilize the `points\_forecast` method inherent to the API. We introduced a bug into this function by using the 'get\_forecasts' method which takes a postal code and country as parameters, but we passed latitude and longitude values instead. (3) Finally, participants were tasked with rectifying a function named 'check\_webpage'. The original intent of this function was to capture all visible elements from a webpage utilizing the Selenium library in Python. Interestingly, we used an obsolete code snippet for this function that was originally generated by ChatGPT.

\boldification{ The second task was …}
\textit{Task 2:} The second task focused on the identification and remediation of code smells \cite{fowler1997refactoring, codesmells}. As per our discussions with the course instructor, it was understood that the students had not yet been formally introduced to the concept of code smells during their coursework. This motivated our design for task 2: which was intended to familiarize participants with the concept of code smells, enabling them to detect their occurrence within the code and implement appropriate fixes. We introduced code smells including global variables, unused imports, dead code (commented out code), lengthy ‘check\_webpage’ function, magic numbers (constants without context), and generalized error handling in the main method (they were allowed to fix code smells in the main method for this task).

\boldification{ Finally, the third task was….}
\textit{Task 3:} In the third task, participants were to commit their contributions to the remote branch and subsequently initiate a Pull Request (PR) from their branch to the base branch. To maintain the integrity of the main branch, we instituted branch protection rules which prevented any modifications in the base branch.

%
\boldification{ Next we selected our analytical lenses for answering our RQs.}
\textit{Selecting our metrics and lenses:} Next we selected metrics and our analytical lenses for answering our RQs.

\boldification{ We assessed cog load using TLX}
\textit{NASA TLX:} To understand how the resources used for the tasks impacted participants' perception of challenge, effort, performance, and frustration in the study, we utilized the NASA Task Load Index (TLX) \cite{hart1988development}. The TLX is a validated and widely used post study survey for measuring cognitive load across six dimensions (mental demand, physical demand, temporal demand, performance, effort, and frustration). We adopted the TLX, utilizing a 21-point Likert scale (aligning with the original scale's standards) extending from 'very low' to 'very high'. 

\boldification{ We adapted Steinmacher et al. method for assessing self reported self efficacy}
\textit{Self-efficacy:} Self-efficacy is a measure reflecting an individual's perceived ability to successfully accomplish a task, and can influence one’s actual ability to complete a task \cite{bandura1986explanatory}. To capture this construct, we used a questionnaire adapted from Steinmacher et al. \cite{steinmacher2016overcoming}, and modified to fit the context of our study. We employed the questionnaire with a 5-point Likert scale (Strongly Disagree, Disagree, Undecided, Agree, Strongly Agree) in a before-after design (same set of questions were posed at the beginning and the end of the study) that allowed us to ascertain the effect of the resources on participants' self-reported levels of self-efficacy.

\boldification{ To assess any AI faults, we need a standardized method. We chose AAR/AI. (Part of it will be shifted to Background)}
\textit{AAR/AI:} We required a lens that end users could use to assess AI faults. But without a detailed standardized process, they may approach assessment in ad hoc ways - leading to wide variations in assessment of the same AI tool only due to variation in their processes. To that end, we employed After-Action Review for AI (AAR/AI) \cite{dodge-aar}, a recent AI assessment process that is focused on supporting humans in gauging AI faults \cite{khanna2022finding}. 

\boldification{ Where is it adopted from?}
AAR/AI is a recent member of the After-Action Review (AAR) family which was originally devised by the U.S. military in the 1970s \cite{morrison1999foundations} as a facilitated debriefing method for assessing human decisions during military training sessions. The AAR method has been used for decades and has subsequently been adapted to different domains including manned unmanned teams \cite{brewer2020assessment} , emergency response \cite{davies2019enhancing, ishak2017slides}, transportation \cite{baird1999learning}, and healthcare \cite{quarles2013experiences, sawyer2013adaptation}. Most of the adaptations have been successful and a meta analysis of 61 studies has found that the AAR method produces a practical moderate effect overall \cite{keiser2021meta}. 

\boldification{ Why did we care? Did studies show that humans assess AI better with AAR/AI?}
AAR/AI is a form of retrospective analysis and reflection to understand what happened, why it happened, and how it can be improved. It is tailor made as an assessment method for a human assessor to judge an AI (review/learn AI’s behavior). Khanna et al. \cite{khanna2022finding} provided empirical evidence that the integration of AAR/AI can aid end users in uncovering not only a significantly larger number of faults, but also in identifying these faults with greater precision. Drawing from Dodge et al. \cite{dodge-aar}, participants using AAR/AI reported that it assisted in better organization of their thoughts and fostered logical reasoning about the AI agent. Moreover, it also encouraged them to reason about the AI and its behavior from a diverse set of perspectives.

\boldification{ How is AAR/AI done and  how does the experimenter facilitate AAR/AI?}
AAR/AI steps are derived from the “DEBRIEF” adaption by Sawyer and Deering \cite{sawyer2013adaptation}. There are seven steps: It starts with Defining the rules, Explaining the objectives of the AI agent, Benchmarking the performance of the agent, Reviewing what was supposed to happen, Identifying what actually happened, Examining why, and finally Formalizing learning. AAR/AI is highly adaptable as it offers flexibility within each step of its process, accommodating customization to suit the specific needs and objectives of AI assessment in different domains. We adapted the AAR/AI steps as follows (Table 2):

\begin{table}[b]
    \footnotesize
    \vspace{-2mm}
    \caption{\label{tab:aar-ai-steps} \small{AAR/AI steps and our adaptations. The Empirical context column explains how we realized the method in our study. Steps 3 to 6 were “inner loop” questions that we repeated for all the three tasks.}}
    \vspace{-2mm}
  \input{table/AARAI-table}
\end{table}

\textit{Defining the rules and explaining the objectives:} Each session commenced with the researcher providing an overview of the interfaces that the participants would be utilizing (GitHub, VS Code), as well as the tasks they would be undertaking. The purpose of the assessment was clearly communicated: ChatGPT was expected to deliver contextual, unambiguous, and accurate information (Steps 1-2, Table 2). In this briefing, the experimental group was explicitly instructed that ChatGPT was to be their sole resource for the tasks. The control group, however, did not undergo the AAR/AI process. 

\textit{The inner loop: What, Why, How:} Following task explanations and before each task initiation, participants answered the question, "What do you think should happen when you use ChatGPT for this task?" Subsequent to each task, they responded to: "What actually happened when you used ChatGPT for this task?", "Why do you think ChatGPT behaved this way?", and "To what extent did you modify ChatGPT’s responses for solving the task? Briefly explain why?" (Steps 3-6, Table 2). The inner loop repeated for all three tasks. For gaining a more concrete understanding of the participants' actions in specific contexts (during each task), we modified Step 6 by substituting "would" with "did" (See sandboxing information). 

\textit{Formalizing learning:} Once all tasks were completed, the formalizing learning stage commenced. Participants were asked: "What went well?", "What did not go well?", and "What could be done differently next time?" (Step 7, Table 2). This step is helpful in showcasing the overall picture after interactions with the AI agent.

\boldification{ Next we needed to link the faults to some guideline violations. There are so many guidelines, but we chose Amershi’s ones (Why). We adapted it as statements as the guidelines were high level advice.}
\textit{Human AI Interaction Guidelines:} In the landscape of human-AI interaction, guidelines can offer invaluable advice on system design and operation. Wright et al.'s \cite{wright2020comparative} exploration of guidelines from three tech giants—Apple, Google, and Microsoft—offered over 200 categorized guidelines, ranging from initial considerations of AI to the curation of the models, the deployment of the AI-powered system, and the human-AI interface. Notably, Wright et al. found that while both Apple’s \cite{AppleGuidelines} and Google’s \cite{GoogleGuidelines} guidelines were developed with the developer in mind, Amershi et al.’s 18 guidelines \cite{amershi2019guidelines} were designed with a keen focus on the user. This distinct approach of user-centric orientation makes Amershi's guidelines particularly relevant to our study as it aligns with our objective to understand the root cause of faults that GenAI makes originating from guideline violations during its design. In our context, we transformed the high-level advice of each guideline into specific statements (retaining the original meaning). Participants were required to rate these statements using a 5-point Likert scale (Strongly Disagree, Disagree, Undecided, Agree, Strongly Agree). Our intent was to identify the potential violations of these guidelines made by ChatGPT during user interaction. The transformations emerged from in-depth discussions within our research team and were successively honed during our sandboxing sessions.

\boldification{ Finally, we also derived intention for future use questions}
\textit{Intention for future use:} To assess the participants' intentions for future use of ChatGPT in the context of software engineering education and tasks, we presented them with three statements: "Based on this experience, I plan to use ChatGPT to learn Software Engineering concepts", "Based on this experience, I plan to use ChatGPT to solve similar kinds of tasks", and "I would recommend ChatGPT to my friends if they need assistance with Software Engineering". The participants were asked to rate their level of agreement with these statements on a 5-point Likert scale, ranging from 'Strongly Disagree' to 'Strongly Agree'.

\boldification{ With this we completed the set, here is a summary of the questions}
Table 3 provides a summary of the questions each group was required to answer at different stages throughout the study.

\begin{table}[b]
    \footnotesize
    \vspace{-2mm}
    \caption{\label{tab:ques-summary} \small{Summary of the questionnaires (see supplementary document) for each group in the study. The questions in each block are listed in their order of appearance. The questionnaires were augmented after the sandboxing session (See sandboxing information).}}
    \vspace{-2mm}
  \input{table/Questionnaire Order}
\end{table}



\boldification{ After the study design, it is important to test whether the design helps us measure what we want. We did sandboxing. We changed from zoom to in lab setting (why) and time boxed tasks (why).}
\textit{Sandboxing:} Over the course of three weeks, we conducted six sandboxing sessions with Computer Science students at the university. The first two sessions were held via Zoom. However, it quickly became apparent that this setup posed several challenges for us, such as prolonged setup times, limitations in our ability to control the environment, and difficulties in library installations. Consequently, we decided to transition from teleconferencing to an in person lab setting. Originally, each session was two hours. However, due to participant fatigue and them spending excessive time on tasks, we adjusted to 80-minute sessions and time-boxed the tasks: Task 1 was allotted 20 minutes, and tasks 2 and 3 had 10 minutes each. This change facilitated on-time conclusions, and time for briefing and questionnaires.

\boldification{ We changed AAR/AI steps a bit based on feedback and observations. Additionally, we reverse coded some items to avoid acquiescence bias. Lastly, we also dropped two guidelines as they were not relevant to our study.}
Our sandboxing phase revealed a challenge in participant engagement with the AAR/AI process: participants found it burdensome, resulting in sparse responses. Echoing a similar concern raised by Dodge et al. \cite{dodge-aar}, we revised steps 3, 4, and 6, employing a mix of open and closed-ended questions to alleviate this issue while still capturing the necessary insights. Step 6 underwent a substantial change based on a sandboxer's feedback. They suggested examining the extent and reasons for modifications in the task, instead of potential future actions. We discussed this recommendation within our research team and reached a consensus that this change would enhance the clarity of our study. Concurring with this feedback, we replaced "would'' with "did" in Step 6, allowing us to better comprehend participants' actions within each task's context. Additionally, we reverse-coded some items with negative connotations (low scores indicating agreement)  in the self-efficacy, intention to use, and Human-AI interaction guideline questionnaires to counter acquiescence bias \cite{baumgartner2001response}, a tendency where participants agree with statements regardless of their content or due to laziness, indifference, or automatic accommodation to a response pattern \cite{podsakoff2003common}. Lastly, all the researchers unanimously agreed to omit Guideline 3 (time services based on context), due to its irrelevance in our specific study with conversational AI (ChatGPT remains idle, unless prompted). Guideline 18 (notify users about changes) was also dropped, given its inapplicability as there were no major ChatGPT updates scheduled during the timeline of the actual study (May 15 - June 2, 2023)).

\boldification{ After our study design was concrete, we set out on a quest for our participants.}
\subsection{Data Collection and Analysis}
\label{subsec:collection-analysis}
\boldification{ We recruited …….}
\textit{Recruitment:} We recruited undergraduate students in Computer Science who were at least 18 years of age and were enrolled in Software Engineering courses at the university. We visited the undergraduate classes in person and briefed them about the study. Interested participants were asked to answer a survey about their demographic information (age, gender, academic level), resources used for software engineering (GitHub, OpenAI), and their experience in programming and software engineering. A total of 41 people responded to the survey.

\boldification{ Our final participants were …… }
\textit{Participants:} After initially filtering out the graduate students and the students who were not familiar with GitHub, we reached out to 39 people asking them to indicate their preferred week, days, and times for the study. We received a total of 30 responses, out of which 26 people indicated availability and only 24 people actually showed up during the study (We later had to disregard 2 participants’ data as their video files were corrupted due to a fault in two lab machines). Of the final 22 participants, 13 self-identified as men and 9 as women. We randomly assigned each participant to one of the two groups: Treatment (with ChatGPT) and Control (without any LLM) while ensuring that there are an equal number of participants in each group. Participant IDs were assigned based on their time of response in an ascending order. The participant demographics are summarized in table 1. As a token of appreciation, students received a \$20 Amazon gift card.

\boldification{ With our participants, we followed this study protocol…}
\textit{Study Protocol:} All studies were in lab sessions at the University lab having up to 3 participants at a time and followed the university IRB protocol. The study proceeded as follows: the participants agreed to an IRB approved informed consent and were briefed about the different stages of the study, then filled out the pre-study questionnaire, then performed the three tasks in the study in a between-subjects design (The control participants could use any online tools other than language models to complete the tasks. The experimental group could only use ChatGPT and were asked to fill the AAR/AI questions before and after each task), and finally filled out the post study questionnaire. The sessions were recorded with participants’ consent and lasted around 80 minutes each. 
Before and after each study session, the browser histories and git branches were deleted to prevent unwarranted advantages and to ensure that all the participants regardless of their group could start the session with exactly the same information. All the participants performed the same tasks in the same order irrespective of their group, and the researcher helped all participants with VS code environment setup. Additionally, the experimental group were briefed about ChatGPT and the primary objective of the language model for the context of the study following AAR/AI steps 1 and 2. 

\boldification{ After data collection, we analyzed our data (how) and found …..}
\rudy{discussion needed for this part}
\textit{Analysis:} To analyze the results, three authors qualitatively analyzed (open coding) AAR/AI open ended questions and identified <> categories of AI faults and <> categories of consequences due to these AI faults. Furthermore, we also identified <> categories of …..
<Need context>


%

==> table/Conseq2.tex <==
\begin{tabular}{p{0.1cm}|p{4.8cm}|p{1.7cm}|p{10cm}}
\hline
 & \textbf{Code: Description} & \textbf{Participants}&\textbf{Exemplary Quotes} \\
\hline
\multirow{2}{*}[-2.2mm]{\rotatebox{90}{\textbf{Uncertainty}}} & \textbf{C1: Uncertainty about correctness}: Users were uncertain about the correctness of the responses/solutions provided by ChatGPT. &PT-1, PT-2, PT-6, PT-10  &``I could not rely on it to tell me when functions exist or not.", ``Some of answers didn’t look right from ChatGPT'', ``I don't think it provided fully correct data, so I am inclined to pick parts only" \\
\cline{2-4}
&\textbf{C2: Uncertainty about how to apply}: Users were unsure/confused about how to apply or use the information provided by ChatGPT. & PT-1, PT-2, PT-3 &``I didn't use ChatGPT's responses since I wasn't sure how to apply them.", ``I'm not super sure why this didn't work. It was fighting me a lot about the whole NOAA thing. Maybe it is not as familiar with this."\\
\hline
\multirow{2}{*}[-3mm]{\rotatebox{90}{\textbf{Reflections}}} & \textbf{C3: ChatGPT was not so helpful}: There were instances where users thought that ChatGPT was not so helpful. & PT-1, PT-5, PT-10, PT-11 &``Everything else I had to do on my own because ChatGPT didn't comprehend enough to help", ``I could not figure out how to fix the import problem, and ChatGPT's suggestions didn't work", ``Having it define or explain ambiguous concepts did not help much", \\
\cline{2-4}
 & \textbf{C4: Self-doubt}: Instances where users doubted themselves suspecting that they might be at fault. & PT-2, PT-4 &``I got confused over suggestions with the weather library, likely I should have provided the full error...And I also may have asked something wrong? Correction wasn't made obvious to me for palindrome", ``I think it gave good ideas for the weather, but I might have missed them initially" \\
% \cline{2-4}
%  & \textbf{Thoughts about future use}: What users thought could be done differently to yield better outcomes in the future. & PT-1, PT-2, PT-3, PT-4, PT-6, PT-10, PT-11 & ``I need to work better about only asking small questions \& identifying the errors by myself. This is easier for ChatGPT to solve.", ``I could have provided more context in my earlier prompts such as background knowledge level \& provide more error output to the agent.", ``More complex tasks with internet access might be better - that way ChatGPT pieces together code", ``I would have liked to be able to ask someone knowledgeable in Python about the imports" \\
\hline
\multirow{3}{*}[-10mm]{\rotatebox{90}{\textbf{Actions}}} & \textbf{C5: Users used their own experience}: Users had to use their own experience to solve certain aspects of the tasks. & PT-1, PT-4, PT-7, PT-10 &``Some answers look evidently wrong or unnecessary. It is important to modify the code based on my experience.", ``Everything else I had to do on my own because ChatGPT didn't comprehend enough to help", ``I used its responses in tandem so I kind of combined them. When it wasn't right, I did it myself." \\
\cline{2-4}
 & \textbf{C6: Users cherry picked solutions}: Users picked parts of solutions provided by ChatGPT that seemed correct. & PT-2, PT-3, PT-5 &``I don't think it provided fully correct data so I am inclined to pick parts only.", ``Some of the things I didn't necessarily agree with but some of it was valid, so I picked \& chose what I liked." \\
\cline{2-4}
 & \textbf{C7: Users modified responses}: Users modified the responses provided by ChatGPT to come up with the correct solution. & PT-6, PT-7, PT-9, PT-10 &``Some code provided by ChatGPT was correct, while some was incorrect and required modifying it", ``I used its responses in tandem so I kind of combined them. When it wasn't right, I did it myself.", ``I made my own modifications and added modified responses from ChatGPT on things I didn't know fully." \\
\hline
\end{tabular}

==> table/Consequences.tex <==
\begin{tabular}{p{0.1cm}|p{5.5cm}|p{11cm}}
\hline
 & \textbf{Code: Description} &\textbf{Exemplary Quotes} \\
\hline
\multirow{2}{*}[-2.2mm]{\rotatebox{90}{\textbf{Uncertainty}}} & \textbf{C1: Uncertainty about correctness}: Users were uncertain about the correctness of ChatGPT's responses/solutions.   &``I could not rely on it to tell me when functions exist or not.", ``Some of answers didn’t look right from ChatGPT'', ``I don't think it provided fully correct data, so I am inclined to pick parts only" \\
\cline{2-3}
&\textbf{C2: Uncertainty about how to apply}: Users were unsure/confused about how to apply/use the information provided by ChatGPT.&``I didn't use ChatGPT's responses since I wasn't sure how to apply them.", ``I'm not super sure why this didn't work. It was fighting me a lot about the whole NOAA thing. Maybe it is not as familiar with this."\\
\hline
\multirow{2}{*}[-3mm]{\rotatebox{90}{\textbf{Reflections}}} & \textbf{C3: ChatGPT was not so helpful}: Instances where users thought that ChatGPT was not so helpful. &``Everything else I had to do on my own because ChatGPT didn't comprehend enough to help", ``I could not figure out how to fix the import problem, and ChatGPT's suggestions didn't work", ``Having it define or explain ambiguous concepts did not help much", \\
\cline{2-3}
 & \textbf{C4: Self-doubt}: Instances where users doubted themselves suspecting that they might be at fault. &``I got confused over suggestions with the weather library, likely I should have provided the full error...And I also may have asked something wrong? Correction wasn't made obvious to me for palindrome", ``I think it gave good ideas for the weather, but I might have missed them initially" \\
\hline
\multirow{3}{*}[-7mm]{\rotatebox{90}{\textbf{Actions}}} & \textbf{C5: Users used their own experience}: Users had to use their own experience to solve certain aspects of the tasks. &``Some answers look evidently wrong or unnecessary. It is important to modify the code based on my experience.", ``Everything else I had to do on my own because ChatGPT didn't comprehend enough to help", ``I used its responses in tandem so I kind of combined them. When it wasn't right, I did it myself." \\
\cline{2-3}
 & \textbf{C6: Users cherry picked solutions}: Users picked parts of solutions provided by ChatGPT that seemed correct. &``I don't think it provided fully correct data so I am inclined to pick parts only.", ``Some of the things I didn't necessarily agree with but some of it was valid, so I picked \& chose what I liked." \\
\cline{2-3}
 & \textbf{C7: Users modified responses}: Users modified the responses provided by ChatGPT to come up with the correct solution.  &``Some code provided by ChatGPT was correct, while some was incorrect and required modifying it", ``I used its responses in tandem so I kind of combined them. When it wasn't right, I did it myself.", ``I made my own modifications and added modified responses from ChatGPT on things I didn't know fully." \\
\hline
\end{tabular}

==> table/Faults.tex <==
%\begin{tabular}{l|l}
\begin{tabular}{p{4cm}|p{13.2cm}}
% {p{2.2cm}|p{1.2cm}|p{4.4cm}}

\hline
\textbf{Code: Description} 
% & \textbf{Participants} 
&\textbf{Exemplary Quotes} \\
\hline
\textbf{F1: Limited advice on niche topics}: ChatGPT struggled to provide expert advice on niche topics. 
% & PT-1, PT-5, PT-9 
&``Well, ChatGPT only was helpful with general info, like git commands or logic issues. It wasn't helpful with niche specifics, like discerning between functions to use in a Python library.", 
``For anything that wasn't super standard, ChatGPT struggled to easily give useful answers.", ``It understood surface-level concepts of git well but not too much depth." \\
\hline
\textbf{F2: Inability to comprehend the problem}: ChatGPT couldn't correctly identify problems and goals. 
% & PT-1, PT-5, PT-6, PT-7, PT-8, PT-10
&``It incorrectly identified nonproblems as problems, and missed actual problems.", ``It doesn't know the exact thing you want it to do despite giving it context.", ``It doesn't fully understand the documentation/interactions of some libraries/functions.", ``It didn't really comprehend the context of the problems and goals" \\
\hline
\textbf{F3: Incomplete assistance}: ChatGPT provided incomplete and partially correct assistance. 
% & PT-1, PT-2, PT-3, PT-6, PT-7, PT-8, PT-9, PT-11
&``I did ask ChatGPT questions about completing the task, but it did not give me answers on how to solve the whole task.", ``Some code provided by ChatGPT was correct, while some was incorrect and required modifying it", ``I could not figure out how to fix the import problem, and ChatGPT's suggestions didn't work" \\
\hline
% \textbf{F4: Can't access relevant information}: ChatGPT did not have access to relevant information needed for assisting the user. & PT-4, PT-6 &``It did not have access to the documentation for the packages we were using, so it hallucinated answers", ``It doesn't fully understand the documentation/interactions of some libraries/functions." \\
% \hline
\textbf{F4: Hallucination}: ChatGPT hallucinated/made up wrong solutions when it did not know the correct solution. 
% & PT-4, PT-9, PT-11 
&``It made up parameters for functions that were unfamiliar", ``It did not have access to the documentation for the packages we were using, so it hallucinated answers", ``It did hallucinate sometimes, said there was a way to use a function in the noaa-sdk that was not possible." \\
\hline
\textbf{F5: Wrong guidance}: Instances where ChatGPT provided wrong guidance to the user. 
% & PT-2, PT-3, PT-4, PT-7, PT-8, PT-9, PT-10, PT-11 
&``The suggestions it gave about code modification are not so helpful. It clearly gave wrong guidance", ``ChatGPT did not have as much knowledge about the NOAA python library, and confidently told me incorrect ways to `fix' my code.", ``Some answers look evidently wrong or unnecessary. It is important to modify the code based on my experience." \\
\hline
\end{tabular}

==> table/Interactions.tex <==
\definecolor{Gray}{gray}{0.85}
    \centering
    \begin{tabular}{l|cc|ccc}
    \hline
        Interactions & Experimental & Control & Estimate & p-value & Cliff's delta \\ \hline
        \rowcolor{Gray}
        Task 1 & 11 & 20 & 21 & \textbf{$0.010^{***}$} & -0.653 \\ 
        \rowcolor{Gray}
        Task 2 & 5 & 2 & 96.5 & \textbf{$0.017^{***}$} & 0.595 \\ 
        \rowcolor{Gray}
        Task 3 & 1 & 4 & 23.5 & \textbf{$0.015^{***}$} & -0.612 \\ 
        \rowcolor{Gray}
        Overall & 19 & 27 & 30 & \textbf{$0.048^{**}$} & -0.504 \\ \hline
    \end{tabular}

==> table/QuestionnaireOrder.tex <==
% \rudy{Can remove the table}
% \boldification{ With this we completed the set, here is a summary of the questions}
% Table 3 summarizes the questionnaires each group answered at different stages throughout the study.

% \begin{table}[ht]
%     \footnotesize
%     \vspace{-2mm}
%     \caption{\label{tab:ques-summary} \small{Summary of the questionnaires (see supplementary document) for each group in the study. The questions in each block are listed in their order of appearance. The questionnaires were improved after the sandboxing sessions (Section \ref{sec:sandbox}).}}
%     \vspace{-2mm}
%   \input{table/QuestionnaireOrder}
%   \vspace{-10px}
% \end{table}

\begin{tabular}{p{1.1cm}p{4.1cm}p{2.2cm}}
    \toprule
    \textbf{Stage} & \textbf{Experimental Group} & \textbf{Control Group} \\
    \midrule
    Pre Study
& Self efficacy questionnaire, Self reported familiarity with AI (enrolled in AI courses/worked on AI projects/limited experience in AI)&
Self-efficacy questionnaire \\
\midrule
    \multicolumn{3}{c}{\textbf{For each task}} \\
    \midrule
   
    Before task & AAR/AI step 3 & None\\
    After task & AAR/AI step 4-6 & None\\
    \midrule
    
    Post Study & AAR/AI step 7, Intention for future use, NASA TLX, Human-AI guideline statements, Self-efficacy questionnaire & NASA TLX, Self-efficacy questionnaire\\
    \bottomrule
  \end{tabular}
















==> table/TLX.tex <==
% \begin{tabular}{|p{1.5cm}|p{0.8cm}|p{1cm}|p{4cm}|}
% \hline
%  & \textbf{Exp} & \textbf{Control} & \textbf{Distribution}\\
% \hline
% Mental & 15 & 14 & \includegraphics[width=4cm,height=1cm]{figures/Mental_boxplot.png}\\
% \hline
% Physical & 1 & 3 & \includegraphics[width=4cm,height=1cm]{figures/Physical_boxplot.png}\\
% \hline
% Temporal & 15 & 15 & \includegraphics[width=4cm,height=1cm]{figures/Temporal_boxplot.png}\\
% \hline
% Performance & 9 & 12 & \includegraphics[width=4cm,height=1cm]{figures/Performance_boxplot.png}\\
% \hline
% Effort & 14 & 14 & \includegraphics[width=4cm,height=1cm]{figures/Effort_boxplot.png}\\
% \hline
% Frustration & 14 & 9 & \includegraphics[width=4cm,height=1cm]{figures/Frustration_boxplot.png}\\
% \hline
% \end{tabular}



% Define a new column type with a grey background
% \newcolumntype{g}{>{\columncolor[gray]{.8}}m{1cm}}

%     \begin{tabular}{l|llllll}
%     \hline
%         Group &Mental&Physi-&Tempo-&Perfor-&Effort&Frustra- \\ 
%        &&cal&ral&mance&&tion\\ \hline
%         Exp & 15 & 1 & 15 & 9 & 14 & 14 \\ 
%         Control & 14 & 3 & 15 & 12 & 14 & 9 \\ \hline
%     \end{tabular}

% \newcolumntype{g}{>{\columncolor[gray]{.8}}m{1.cm}}
\definecolor{Gray}{gray}{0.85}
    \centering
    \begin{tabular}{l|cc|ccc}
    \hline
        Dimension & Experimental & Control & Estimate & p-value & Cliff's delta $(\delta)$ \\ \hline
        Mental & 15 & 14 & 47 & 0.388 & -0.223 \\ 
        Physical & 1 & 3 & 51.5 & 0.557 & -0.149 \\ 
        Temporal & 15 & 15 & 64.5 & 0.817 & 0.066 \\ 
        Performance & 9 & 12 & 45.5 & 0.339 & -0.248 \\ 
        Effort & 14 & 14 & 45.5 & 0.337 & -0.248 \\ 
        \rowcolor{Gray}
        \textbf{Frustration} & 14 & 9 & 101 & \textbf{$0.008^{***}$} & \textbf{0.669} \\ \hline
    \end{tabular}
    



    












==> table/Task_Performance.tex <==
\definecolor{Gray}{gray}{0.85}
    \centering
    \begin{tabular}{l|cc|ccc}
    \hline
        Scores & Experimental & Control & Estimate & p-value & Cliff's delta \\ \hline
        Task 1 & 1 & 2 & 40 & 0.160 & -0.339 \\ 
        Task 2 & 1 & 0 & 86 & 0.078 & 0.421 \\ 
        Task 3 & 2 & 2 & 71.5 & 0.303 & 0.182 \\ 
        Overall & 4 & 4 & 71 & 0.507 & 0.174 \\ \hline
    \end{tabular}

==> table/conseq3.tex <==
\begin{tabular}{p{0.1cm}|p{2.8cm}|p{4.5cm}}
\hline
 & \textbf{Code}&\textbf{Description} \\
\hline
\multirow{2}{*}[-0.5mm]{\rotatebox{90}{\textbf{Uncertainty}}} & \textbf{C1: Uncertainty about correctness} & Users were uncertain about the correctness of ChatGPT's responses/solutions. \\
\cline{2-3}
&\textbf{C2: Uncertainty about how to apply} & Users were unsure/confused about how to apply/use the information provided by ChatGPT.\\
\hline
\multirow{2}{*}[-1.2mm]{\rotatebox{90}{\textbf{Reflections}}} & \textbf{C3: ChatGPT was not so helpful} & Instances where users thought that ChatGPT was not so helpful. \\
\cline{2-3}
 & \textbf{C4: Self-doubt}& Instances where users doubted themselves suspecting that they might be at fault. \\
\hline
\multirow{3}{*}[-5mm]{\rotatebox{90}{\textbf{Actions}}} & \textbf{C5: Users used their own experience}& Users had to use their own experience to solve certain aspects of the tasks. \\
\cline{2-3}
 & \textbf{C6: Users cherry picked solutions} & Users picked parts of solutions provided by ChatGPT that seemed correct.\\
\cline{2-3}
 & \textbf{C7: Users modified responses} & Users modified the responses provided by ChatGPT to come up with the correct solution.  \\
\hline
\end{tabular}
